Collaborative Learning of Discrete Distributions under Heterogeneity and Communication Constraints

In modern machine learning, users often have to collaborate to learn the distribution of the data. Communication can be a significant bottleneck. Prior work has studied homogeneous users -- i.e., whose data follow the same discrete distribution -- and has provided optimal communication-efficient methods for estimating that distribution. However, these methods rely heavily on homogeneity, and are less applicable in the common case when users' discrete distributions are heterogeneous. Here we consider a natural and tractable model of heterogeneity, where users' discrete distributions only vary sparsely, on a small number of entries. We propose a novel two-stage method named SHIFT: First, the users collaborate by communicating with the server to learn a central distribution; relying on methods from robust statistics. Then, the learned central distribution is fine-tuned to estimate their respective individual distribution. We show that SHIFT is minimax optimal in our model of heterogeneity and under communication constraints. Further, we provide experimental results using both synthetic data and $n$-gram frequency estimation in the text domain, which corroborate its efficiency.

==> bmacros.tex <==
%% Version: 2017-04-09
%% common packages
\usepackage{hyperref}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{color}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{wasysym}
\usepackage{lmodern} % to avoid font size not available warning
\usepackage{textcomp} % to avoid font warning for textbullet used in \item
\usepackage{wasysym} % useful symbols
\usepackage{dashbox} % for use of dashd box \dbox{...}
\usepackage{mathtools} % for \DeclarePairedDelimiter below
\mathtoolsset{showonlyrefs} % only the used numbers will appear
\usepackage{tabto}  % for \NumTabs{3} and \tab commands
%\usepackage{mathabx} % for \vvvert matrix norm
\usepackage[ruled,vlined]{algorithm2e}

%% to reduce footnote font size
\usepackage{etoolbox}
\makeatletter
\patchcmd{\@makefntext}{\insertfootnotetext{#1}}{\insertfootnotetext{\scriptsize#1}}{}{}
\makeatother

%% begin and end backup slides
\newcommand{\backupbegin}{
   \newcounter{framenumberappendix}
   \setcounter{framenumberappendix}{\value{framenumber}}
}
\newcommand{\backupend}{
   \addtocounter{framenumberappendix}{-\value{framenumber}}
   \addtocounter{framenumber}{\value{framenumberappendix}}
}

%% one-page section title and subsection title, which skip and hide page numbers
\newcommand{\sectiononepage}[1]{
  \section{#1}
  \begin{frame}[plain,noframenumbering]\begin{center}\begin{Large}\textbf{#1}\end{Large}\end{center}\end{frame}
}
\newcommand{\subsectiononepage}[1]{
  \subsection{#1}
  \begin{frame}[plain,noframenumbering]\begin{center}\begin{Large}\textbf{#1}\end{Large}\end{center}\end{frame}
}

%% macros for commenting
\usepackage[normalem]{ulem} % to use \sout
\newcommand{\remove}[1]{{\color{Gray}\sout{#1}}}
\newcommand{\revise}[1]{{\color{blue}#1}}
\newcommand{\commwy}[1]{{\color{red}(wy: #1)}} % Wotao Yin
\newcommand{\cut}[1]{{}}  % text cut out

%% check and cross marks
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%% check mark
\newcommand{\xmark}{\ding{55}}%% cross mark

%% blue equation box
\usepackage{empheq}
\definecolor{myblue}{rgb}{.8, .8, 1}
\newcommand*\mybluebox[1]{%
\colorbox{myblue}{\hspace{1em}#1\hspace{1em}}}

%% template for beamer
\makeatletter
  \@ifclassloaded{article} % check if article is used as the documentclass
    {}% true code
    {
      %% to allow citation as footnote
      \usepackage{natbib}
      \newcommand{\citesmall}[2][]
      {
         \ifthenelse{\equal{#1}{}}
         {\begin{small}\citep{#2}\end{small}}
         {\begin{small}\citep[#1]{#2}\end{small}}
      }
      \newcommand{\citefootnote}[2][]
      {
        \footnote{
          \ifthenelse{\equal{#1}{}}
          {\begin{small}\citep{#2}\end{small}}
          {\begin{small}\citep[#1]{#2}\end{small}}
        }
      }

      %% beamer modifier
      \mode<presentation>
      {
        % page number
        %\setbeamertemplate{footline}{\insertframenumber/\inserttotalframenumber}
        \setbeamertemplate{footline}[frame number]

        % background and theme
        \setbeamertemplate{background canvas}[vertical shading][bottom=white!10,top=white!10]
        \usetheme{default}

        % section in table of contents has numbers
        \setbeamertemplate{sections/subsections in toc}[sections numbered]

        % no navigation bottoms
        \setbeamertemplate{navigation symbols}{}

        % itemize, black bullet, %150 spacing between items using "witemize"
        \setbeamertemplate{itemize items}[circle]
        \setbeamercolor{itemize item}{fg=black}
        \setbeamercolor{enumerate item}{fg=black}
        \setbeamercolor{itemize subitem}{fg=black}
        \setbeamercolor{enumerate subitem}{fg=black}
        \newenvironment{witemize}{\itemize\addtolength{\itemsep}{0.4\baselineskip}}{\enditemize}

        % itemize enumerate use normal sized texts
        \setbeamertemplate{itemize/enumerate body begin}{\normalsize}
        \setbeamertemplate{itemize/enumerate subbody begin}{\normalsize}
        \setbeamertemplate{itemize/enumerate subsubbody begin}{\normalsize}

        % block, black over gray with no shadow
        \setbeamertemplate{blocks}[rounded][shadow=false]
        \setbeamercolor{block title}{fg=black,bg=gray!40}
        \setbeamercolor{block body}{fg=black,bg=gray!10}

        % frametitle, bold, black, centered
        \setbeamertemplate{frametitle}[default][center]
        \setbeamercolor{frametitle}{fg=black}
        \setbeamerfont{frametitle}{shape=\bfseries}

        % line spacing
        \linespread{1.2}

        \setlength{\parskip}{\smallskipamount}

        % make beamer notes itemized instead of enumerated
        \AtBeginNote{%
          \let\enumerate\itemize%
          \let\endenumerate\enditemize%
        }

        % make the note page simpler
        \setbeamertemplate{note page}[compressed]
        \setbeamercolor{note page}{bg=white}
      }
    } % false code (above)
\makeatother%

%% macros for letters

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\valpha}{{\boldsymbol \alpha}}
\newcommand{\vbeta}{{\boldsymbol \beta }}
\newcommand{\vgamma}{{\boldsymbol \gamma}}
\newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vsigma}{{\boldsymbol \sigma}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bb}{{\boldsymbol{b}}}
\newcommand{\bc}{{\boldsymbol{c}}}
\newcommand{\bd}{{\boldsymbol{d}}}
\newcommand{\be}{{\boldsymbol{e}}}
\newcommand{\bldf}{{\boldsymbol{f}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bi}{{\boldsymbol{i}}}
\newcommand{\bj}{{\boldsymbol{j}}}
\newcommand{\bk}{{\boldsymbol{k}}}
\newcommand{\bl}{{\boldsymbol{l}}}
\newcommand{\bm}{{\boldsymbol{m}}}
\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\bo}{{\boldsymbol{o}}}
\newcommand{\bp}{{\boldsymbol{p}}}
\newcommand{\bq}{{\boldsymbol{q}}}
\newcommand{\br}{{\boldsymbol{r}}}
\newcommand{\bs}{{\boldsymbol{s}}}
\newcommand{\bt}{{\boldsymbol{t}}}
\newcommand{\bu}{{\boldsymbol{u}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bz}{{\boldsymbol{z}}}

\newcommand{\bA}{{\boldsymbol{A}}}
\newcommand{\bB}{{\boldsymbol{B}}}
\newcommand{\bC}{{\boldsymbol{C}}}
\newcommand{\bD}{{\boldsymbol{D}}}
\newcommand{\bE}{{\boldsymbol{E}}}
\newcommand{\bF}{{\boldsymbol{F}}}
\newcommand{\bG}{{\boldsymbol{G}}}
\newcommand{\bH}{{\boldsymbol{H}}}
\newcommand{\bI}{{\boldsymbol{I}}}
\newcommand{\bJ}{{\boldsymbol{J}}}
\newcommand{\bK}{{\boldsymbol{K}}}
\newcommand{\bL}{{\boldsymbol{L}}}
\newcommand{\bM}{{\boldsymbol{M}}}
\newcommand{\bN}{{\boldsymbol{N}}}
\newcommand{\bO}{{\boldsymbol{O}}}
\newcommand{\bP}{{\boldsymbol{P}}}
\newcommand{\bQ}{{\boldsymbol{Q}}}
\newcommand{\bR}{{\boldsymbol{R}}}
\newcommand{\bS}{{\boldsymbol{S}}}
\newcommand{\bT}{{\boldsymbol{T}}}
\newcommand{\bU}{{\boldsymbol{U}}}
\newcommand{\bV}{{\boldsymbol{V}}}
\newcommand{\bW}{{\boldsymbol{W}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bY}{{\boldsymbol{Y}}}
\newcommand{\bZ}{{\boldsymbol{Z}}}

\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\blambda}{{\boldsymbol{\lambda}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\renewcommand{\bell}{{\boldsymbol{\ell}}}

\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}

\newcommand{\rint}{{\mathrm{ri}}}

%% macros for math notions and operators

% \newcommand{\EE}{\mathbb{E}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\renewcommand{\SS}{{\mathbb{S}}}
\newcommand{\SSp}{\mathbb{S}_{+}}
\newcommand{\SSpp}{\mathbb{S}_{++}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{{\mathbf{1}}}
\newcommand{\Null}{{\mathrm{Null}}}
\newcommand{\dist}{{\mathrm{dist}}}
\newcommand{\Co}{{\mathbf{Co}}}

\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\epi}{{\mathrm{epi}}} % epigraph
\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}}
\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mini}{minimize}
\DeclareMathOperator*{\maxi}{maximize}
\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}
\newcommand{\fwd}{{\mathbf{fwd}}}
\newcommand{\prox}{{\mathbf{prox}}}
\newcommand{\refl}{{\mathbf{refl}}}
\newcommand{\proj}{{\mathbf{proj}}}
\newcommand{\solve}{\stackrel{\mathrm{solve}}\longleftarrow}
\newcommand{\st}{{\quad\mathrm{s.t.}}}
\newcommand{\St}{{\quad\mathrm{subject~to}}}
\newcommand{\pt}{{\textbullet\ }}

\newcommand{\vvvert}{{\vert\kern-0.25ex\vert\kern-0.25ex\vert}}

% --- OpSplitting specific macro ---
\newcommand{\Fix}{{\mathrm{Fix}}}
\newcommand{\tnabla}{{\widetilde{\nabla}}}
\newcommand{\TFBS}{T_{\mathrm{FBS}}}
\newcommand{\TBFS}{T_{\mathrm{BFS}}}
\newcommand{\TFBFS}{T_{\mathrm{FBFS}}}
\newcommand{\TPRS}{T_{\mathrm{PRS}}}
\newcommand{\TDRS}{T_{\mathrm{DRS}}}
\newcommand{\TDYS}{T_{\mathrm{DYS}}}
\newcommand{\TPRSl}{T^\lambda_{\mathrm{PRS}}}
\newcommand{\kbest}{{k_{\mathrm{best}}}}

\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}  % inner product
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}    % ceil function
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor} % floor function

%% macros for theorem-like environments

\makeatletter
  \@ifclassloaded{article} % check if article is used as the documentclass
    {
      \newtheorem{theorem}{Theorem}
      \newtheorem{definition}{Definition}
      \newtheorem{example}{Example}
    }% true code
    {} % false code
\makeatother%z

\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remark}{Remark}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proof}{Proof}
\newtheorem{proposition}{Proposition}

%\newtheorem{example}[remark]{Example}

